KVLinC : KV Cache Quantization with Hadamard Rotation and Linear Correction

Quantizing the key-value (KV) cache is a promising strategy for improving the inference efficiency of large language models (LLMs). However, aggressive quantization to very low precision (e.g., 2 bits) introduces significant errors in the stored key and value tensors, which propagate through the dot-product attention mechanism and ultimately degrade generation quality. To address this, we propose KVLinC, a framework to mitigate attention errors introduced by KV cache quantization in the extreme low-precision regime. KVLinC combines a Hadamard rotation, which reduces quantization error in values, with lightweight linear correction adapters that explicitly compensate for errors introduced by quantized keys. Across extensive evaluations on the LLaMA, Qwen2.5, and Qwen3 model families, KVLinC consistently matches or surpasses strong baselines while achieving higher KV-cache compression. Furthermore, we implement a custom attention kernel that results in upto 2.55x faster inference compared to Flash Attention baseline, enabling efficient long-context LLM inference.

==> iclr2026/tables/combined_tables_paper.tex <==

\begin{figure}[t]
  \centering
  % ---- left: TABLE ----
  \begin{minipage}[t!]{0.5\textwidth}
    \centering
    \captionof{table}{Performance with applying Hadamard rotation and linear correction in isolation. $\uparrow$ higher is better, $\downarrow$: lower is better.}
    \label{tab:main_results}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c}
    \hline
    \textbf{Model} & \textbf{Method} & \textbf{Wikitext} & \textbf{GSM8K-5shot} \\ \hline
    \multirow{4}{*}{Llama-3.1-8B} & KIVI & 7.8 & 34.1 \\
     & KIVI + LinC & 7.3 & 38.4 \\
     & Q\_c(K), V\_t(VH) & 7.2 & 36.9 \\
     & KVLINC & 7.1 & 40.9 \\ \hline
    \multirow{4}{*}{Llama-3.1-3B} & KIVI & 11.0 & 11.8 \\
     & KIVI + LinC & 9.8 & 14.5 \\
     & Q\_c(K), V\_t(VH) & 9.7 & 13.9 \\
     & KVLINC & 9.4 & 15.9 \\ \hline
    \end{tabular}
    }
  \end{minipage}%
  \hfill%
  \begin{minipage}[!t]{0.45\textwidth}
    \centering
    \small
    \captionof{table}{\% PPL improvement vs.\ KIVI by decoder block (higher is better).}
    \label{tab:block-impr-table}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ccc}
    \toprule
    \multirow{2}{*}{Decoder block} & \multicolumn{2}{c}{Improvement (\%)} \\
    % \cmidrule(lr){2-3}
    & {Qwen 2.5 1.5B} & {Qwen 3 1.7B base} \\
    \midrule
    [0--9]   & 7.96 & 3.03 \\
    [10--18] & 4.35 & 2.44 \\
    [19--27] & 2.73 & 1.20 \\
    [0--13]  & 10.55 & 3.75 \\
    [14--27] & 4.29 & 2.33 \\
    [0--28]  & 16.82 & 5.27 \\
    \bottomrule
    \end{tabular}
    }
    \label{fig:block-gain}
  \end{minipage}%
\end{figure}

==> iclr2026/tables/different_components.tex <==
\begin{table}[t!]
\centering
\caption{Main results. $\uparrow$ higher is better, $\downarrow$: lower is better.}
\label{tab:main_results}
\resizebox{0.55\textwidth}{!}{
\begin{tabular}{c|c|c|c}
\hline
\textbf{Model} & \textbf{Method} & \textbf{Wikitext} & \textbf{GSM8K-5shot} \\ \hline
\multirow{4}{*}{Llama-3.1-8B} & KIVI & 7.8 & 34.1 \\
 & KIVI + LinC & 7.3 & 38.4 \\
 & Q\_c(K), V\_t(VH) & 7.2 & 36.9 \\
 & KVLINC & 7.1 & 40.9 \\ \hline
\multirow{4}{*}{Llama-3.1-3B} & KIVI & 11.0 & 11.8 \\
 & KIVI + LinC & 9.8 & 14.5 \\
 & Q\_c(K), V\_t(VH) & 9.7 & 13.9 \\
 & KVLINC & 9.4 & 15.9 \\ \hline
\end{tabular}
}
\end{table}
